Non-Parametric Few-Shot Learning for Word Sense Disambiguation

Word sense disambiguation (WSD) is a long-standing problem in natural language processing. One significant challenge in supervised all-words WSD is to classify among senses for a majority of words that lie in the long-tail distribution. For instance, 84% of the annotated words have less than 10 examples in the SemCor training data. This issue is more pronounced as the imbalance occurs in both word and sense distributions. In this work, we propose MetricWSD, a non-parametric few-shot learning approach to mitigate this data imbalance issue. By learning to compute distances among the senses of a given word through episodic training, MetricWSD transfers knowledge (a learned metric space) from high-frequency words to infrequent ones. MetricWSD constructs the training episodes tailored to word frequencies and explicitly addresses the problem of the skewed distribution, as opposed to mixing all the words trained with parametric models in previous work. Without resorting to any lexical resources, MetricWSD obtains strong performance against parametric alternatives, achieving a 75.1 F1 score on the unified WSD evaluation benchmark (Raganato et al., 2017b). Our analysis further validates that infrequent words and senses enjoy significant improvement.

==> 3_task.tex <==
\section{Task}
\label{sec:task}
Given an input sentence $x = x_1, x_2, \ldots, x_n$, the goal of \ti{all-words} word sense disambiguation (WSD) task is to assign a sense $y_i$ for every word $x_i$ so that $y_i \in \mathcal{S}_{x_i} \subset \mathcal{S}$ for a given sense inventory such as WordNet. In practice, not all the words in a sentence are annotated, and only a subset of positions are identified $\mathcal{I} \subseteq \{1, 2, \ldots, n\}$ to be disambiguated. The goal is to predict $y_i$ for $i \in \mathcal{I}$.
We regard all the instances of a word $w \in \mathcal{W}$ as a classification task $\mathcal{T}_w$, since only all the instances of word $w$ share the output label set $\mathcal{S}_{w}$\footnote{Here we use word $w$ for simplicity. In the WSD dataset, a word is the combination of its stem and part-of-speech tag.}. We define input $\bar{x} = (x, t)$ where $x$ is an input sentence, and $1 \leq t \leq n$ is the position of the target word and the output is $y_t$ for the $t$-th word $x_t$ in $x$. A WSD system is a function $f$ such that $y = f(\bar{x})$. To tackle the long tail problem, we group the training instances by word $w$: $\mathcal{A}(w) = \{((x^{(i)}, t^{(i)}), y^{(i)}): x^{(i)}_{t^{(i)}} = w\}_{i=1}^{\mathcal{N}(w)}$ where $\mathcal{N}(w)$ is the number of training instances for $\mathcal{T}_w$. We will demonstrate in Section~\ref{sec:method} the training algorithm to learn explicitly by task as oppose to mixing all tasks in regular multi-task training paradigm.

==> archive/abstract_intro_comments.tex <==
\danqi{Thoughts on the title? The term non-parametric few-shot learning is from \href{https://cs330.stanford.edu/slides/cs330_nonparametric_2020.pdf}{this}. You can think of ideas along the line of ``learning to model the tail''.}

\danqi{1) Don't mention $N$-way $K$-shot at all in this paper. Our setup is very different from that. 2) Don't use ``task and class distributions''. Nobody knows what ``task'' refers to at the beginning.

Here are my suggestions on the flow/story for both abstract and introduction  (rephrase the sentences):
\begin{itemize}
    \item
        Supervised WSD is an important and well-studied problem.
    \item
        It poses interesting learning challenges because 1) a majority of words have very few training examples; 2) the distribution of senses is highly imbalanced (e.g., predicting the most frequent sense gives XX accuracy).
    \item
        Recent approaches focus on parameteric models and tackles this problem through parameter sharing and learn all the words mixedly (both frequent and infrequent).
    \item
        In this paper, we propose a simple non-parametric few-shot learning approach to address this data scarcity issue. Through episodic sampling and metric learning between examples of the same class, our approach is able to effectively transfer knowledge from frequent words to infrequent words.
    \item
        Without resorting to any knowledge resources (gloss or semantic structure of senses), our approach can achieve XX and it is especially effective on infrequent words and senses.
\end{itemize}
}

==> archive/cross_encoder.tex <==
\begin{equation*}
\begin{split}
    \bert{BERT}(x, x') = \{\bert{CLS}: \mf{h}_{\bert{[CLS]}}, 1: \mf{h}_{x_1}, \ldots, \\ n: \mf{h}_{x_n}, \bert{SEP}: \mf{h}_{\bert{[SEP]}}, 1': \mf{h}_{x'_1}, \ldots, \\ n': \mf{h}_{x'_{n'}}, \bert{SEP}': \mf{h}_{\bert{[SEP]}}\}
\end{split}
\end{equation*}
for a pair of sentences: $x = x_1, \ldots, x_n$ and $x' = x'_1, \ldots, x'_{n'}$.

\paragraph{Cross-encoder}
We concatenate $x$ and $x'$ and pass the sequence to one encoder and it returns a similarity score. It has been demonstrated that cross-encoder has a great advantage in capturing the dependencies between the two input sequences through the self-attention layers \cite{huang2019glossbert, gao2019fewrel}.
Specifically, we compute the score: $s(\bar{x}, \bar{x}') = \mf{w}^{\intercal} \Big[\bert{BERT}(x, x')[t]; \bert{BERT}(x, x')[t'] \Big]$, where $\mf{w}$ is learnable parameters.
%\begin{align}
%s(\bar{x}, \bar{x}') = \mf{w}^{\intercal} \Big[\bert{BERT}(x, x')[t]; \bert{BERT}(x, x')[t'] \Big],
%\end{align}

For each task $w$, $\lvert \supportset(w) \rvert \times \lvert \queryset(w) \rvert$ scores are computed for every support-query pair: $s(\bar{x}, \bar{x}')$, $\forall \bar{x} \in \supportset(w)$ and $\bar{x}' \in \queryset(w)$. Given a query example $(\bar{x}', y') \in \queryset(w)$, the scores of the same sense $j$ is averaged to calculate the sense probability given the query:
\begin{align*}
r_j = \frac{1}{\lvert \supportset_j(w) \rvert} \sum_{(\bar{x}, y) \in \supportset_j(w)} s(\bar{x}, \bar{x}').
\end{align*}
The probability of predicting sense $j$ is computed by:
\begin{align*}
p(y=j \mid \bar{x}') = \frac{\exp(r_j)}{\sum_{k} \exp(r_k)}.
\end{align*}

==> archive/gloss_info.tex <==
\paragraph{Gloss Information}
Gloss is shown to be effective when embedded as sense representation. The semantic overlap between glosses can help the model generalize to unseen senses.
We use gloss to further improve our sense representation on top of the embedded supports. A gloss is a sequence $g = g_1, g_2, \ldots, g_m$ and is available through WordNet for sense $j$.
We use a separate BERT encoder to embed gloss $g$ and take the heading $\bert{[CLS]}$ as the gloss representation: $\glossenc(g) = \bert{BERT}(g)[0]$. A comined score for sense $j$ is computed by:
\begin{align*}
\begin{split}
s(\bar{x}, \bar{x}') = -d(\vec{c}_j, \contextenc(\bar{x}')) - d(\mf{W} \glossenc(g), \contextenc(\bar{x}')),
\end{split}
\end{align*}
where $\mf{W}$ is a linear layer that maps the gloss representation to the same space as the context encoded representations, and $\vec{c}_j$ is the prototype representation in Equation~\ref{proto}. The probability is calculated as in Equation~\ref{softmax}. \howard{Need to clean up notation again. Maybe need to merge distance and score.}

==> tables/breakdown.tex <==
\begin{table}[th!]
{
\begin{tabular}{p{1.7cm}c|ccc}
\toprule
  Word Freq & BEM & BERT-linear & Ours \\
\midrule
$(0, 10]$      & \textbf{72.7} & 54.5 & 63.6 \\
$(10, 20]$     & 76.9  & 69.2 & \textbf{79.5} \\
$(20, 50]$     & \textbf{73.4}  & 70.3 & 67.5 \\
$(50, 100]$    & 68.1 & \textbf{72.3} & \textbf{72.3} \\
$(100, 200]$   & \textbf{69.8}  & 63.5 & 63.5 \\
$(200, 400]$   & 74.5  & 74.5 & \textbf{78.4} \\
$(400, 1000]$  & \textbf{66.7} & 60.0 & 62.2 \\
$(1000, 2200]$ & 65.0 & 55.0 & \textbf{70.0} \\
FULL           & \textbf{71.3} & 66.0 & 69.2 \\
%SE07 (F1)      & 73.4 & 68.6 & 71.4 \\
\bottomrule
\end{tabular}
}
\caption{Accuracy on the development set (SE07) grouped by the word frequency (\# of training examples in SemCor). Single-sense words and unseen words are skipped in the FULL subset. BEM and BERT-linear are reproduced with the code and implementation in~\citep{blevins2020moving}. \howard{will move to figure}}
\label{table:dev_acc_by_word_freq}
\end{table}

\begin{table}[th!]
{
\begin{tabular}{p{1.7cm}c|ccc}
\toprule
  Sense Freq & BEM & BERT-linear & Ours \\
\midrule
$(0, 2]$     & \textbf{48.6} & 22.9 & 37.1\\
$(2, 5]$     & 48.8 & 48.8 & \textbf{63.4}\\
$(50, 10]$   & 76.3 & 71.1 & \textbf{78.9}\\
$(10, 20]$   & 76.5 & \textbf{78.7} & 68.1\\
$(20, 40]$   & 74.0 & 72.0 & 72.0\\
$(40, 80]$  & \textbf{81.6} & 77.6 & 79.6\\
$(80, 200]$ & \textbf{87.8} & 81.6 & 85.7\\
$(200, 2000]$ & \textbf{100.0} & 97.6 & 97.6\\
FULL & \textbf{71.3} & 66.0 & 69.2\\
\bottomrule
\end{tabular}
}
\caption{Accuracy on the development set (SE07) grouped by the sense frequency (\# of training examples in SemCor). Single-sense words and unseen words are skipped in the FULL subset. BEM and BERT-linear are reproduced with the code and implementation in~\citep{blevins2020moving}. \howard{will move to figure}}
\label{table:dev_acc_by_word_freq}
\end{table}


==> tables/mfs_lfs.tex <==
\begin{table}[th!]
\begin{tabular}{p{2.0cm}|cc}
\toprule
%   & \multirow{2}{*}{MFS} & \multirow{2}{*}{LFS} & \multicolumn{2}{c}{Zero-shot} \\
%   & & & Words & Senses \\
   & MFS & LFS \\
\midrule
   WordNet S1 & 100.0 & 0.0 \\
   BERT-linear & 94.9 & 37.0\\

   EWISE & 93.5 & 31.2\\
   BEM & 94.1 & 52.6\\
   Ours & 93.7 & 40.1\\
%   Ours (gloss) & XX & XX & - & - \\
\bottomrule
\end{tabular}
\caption{caption}
\label{table:mfs_lfs}
\end{table}

==> tables/sampling_strategy.tex <==
%!TEX root = ../main.tex
\begin{table}[th!]
\footnotesize
\begin{tabular}{l c}
\toprule
   Sampling & Dev F1 \\
\midrule
   Original ($P_o$) & 66.8\\
   Balanced ($P_b$) & 69.0\\
\bottomrule
\end{tabular}
\caption{Ablation on the sampling strategy. The ablated system hyperparameters are provided in ~\ref{sec:appendix}.}
\label{table:sampling_strategy}
\end{table}


==> tables/zero_shot.tex <==
%!TEX root = ../main.tex

\begin{table}[th!]
\begin{tabular}{p{2.0cm}|cccc}
\toprule
   & \multirow{2}{*}{MFS} & \multirow{2}{*}{LFS} & \multicolumn{2}{c}{Zero-shot} \\
   & & & Words & Senses \\

\midrule
   WordNet S1 & 100.0 & 0.0 & 84.9 & 53.9 \\
   BERT-linear & 94.9 & 37.0 & 84.9 & 53.6 \\

   EWISE & 93.5 & 31.2 & 91.0 & - \\
   BEM & 94.1 & 52.6 & 91.2 & 68.9 \\
   Ours & 93.7 & 40.1 & - & - \\
%   Ours (gloss) & XX & XX & - & - \\
\bottomrule
\end{tabular}
\caption{caption}
\label{table:mfs_lfs_zeroshot}
\end{table}

